A Multi-cut Formulation for Joint Segmentation and Tracking of Multiple Objects

Recently, Minimum Cost Multicut Formulations have been proposed and proven to be successful in both motion trajectory segmentation and multi-target tracking scenarios. Both tasks benefit from decomposing a graphical model into an optimal number of connected components based on attractive and repulsive pairwise terms. The two tasks are formulated on different levels of granularity and, accordingly, leverage mostly local information for motion segmentation and mostly high-level information for multi-target tracking. In this paper we argue that point trajectories and their local relationships can contribute to the high-level task of multi-target tracking and also argue that high-level cues from object detection and tracking are helpful to solve motion segmentation. We propose a joint graphical model for point trajectories and object detections whose Multicuts are solutions to motion segmentation {\it and} multi-target tracking problems at once. Results on the FBMS59 motion segmentation benchmark as well as on pedestrian tracking sequences from the 2D MOT 2015 benchmark demonstrate the promise of this joint approach.

==> introduction.tex <==
Several problems in computer vision, such as image segmentation or motion segmentation in video, are traditionally approached in a low-level, bottom-up way while other tasks like object detection, multi-target tracking, and action recognition often require previously learned model information and are therefore traditionally approached from a high-level perspective.

In this paper, we propose a joint formulation for one such classical high-level problem (multi-target tracking) and a low-level problem (moving object segmentation).

Multi-target tracking and motion segmentation are both active fields in computer vision \cite{Segal_2013_ICCV,Huang:2008:ROT,WojekECCV10,AndrilukaCVPR2010,FragkiadakiECCV12,Zamir:2012:GMC,WojekPAMI2013,Henschel:2014:EMP,tang14ijcv,shiICCV2013,Ochs14,Dragon2014,Ji2014,keuper15a}.
These two problems are clearly related in the sense that their goal is to determine those regions that belong to the same moving object in an image sequence.

We argue that these interrelated problems can and should be addressed jointly so as to leverage the advantages of both.
In particular, the low-level information contained in point trajectories and in their relation to one another form important cues for the high-level task of multi-target tracking. They carry the information where single, well localized points are moving and can thus help to disambiguate partial occlusions and motion speed changes, both of which are key challenges for multi-target tracking. For motion segmentation, challenges are presented by (1) articulated motion, where purely local cues lead to over-segmentation and (2) coherently moving objects where motion cues cannot tell the objects apart. High level information from an object detector or even an object tracking system is beneficial as it provides information about the rough object location, extent, and possibly re-identification after occlusion.

Ideally, employing such pairwise information between detections may replace higher-order terms on trajectories as proposed in \cite{Ochs12}. While it is impossible to tell two rotational or scaling motions apart from only pairs of trajectories, pairs of detection bounding boxes contain enough points to distinguish their motion. With sufficiently complex detection models, even articulated motion can be disambiguated.

%The joint formulation enriches the model capacity and reduces the model complexity.
%  More specifically, in a graph which has only pairwise terms between the detection nodes,
%  one can only compute the speed between two detections.
%  In case of objects with different speeds, triple terms have to be introduced to model the motion similarity. However, pairwise terms between trajectories can already provide this information.
%  On the motion segmentation side, to model scaling or in-plane rotational motion, triple terms between three trajectories are needed \cite{Ochs12}. However, pairwise similarity measures for detection bounding boxes can be computed efficiently in a scale invariant and, if beneficial, in a rotation invariant or robust way.
% Thus, in the joint graph, the pairwise terms between trajectories and detections can mediate the higher order motion relations between motion trajectories and bounding boxes.
%There are also differences. While the main applications for motion segmentation, such as action tube proposals \cite{actiontubes} for action recognition \cite{actiontubes,gkioxari2015wholesandparts}, require the motion segmentations to be spatially highly accurate and favor precision over recall, multi-target tracking rather focuses on not missing a moving object. The exact localization of object boundaries within a bounding box is usually secondary. Much interest is, however, paid on high-level information in order to avoid e.g. ID-switches.
To leverage high-level spatial information as well as low-level motion cues in both scenarios, we propose a unified graphical model in which multi-target tracking and motion segmentation are both cast in one graph partitioning problem.
%The result of this approach are spatially clustered and temporally tracked detections that are linked to partitioned motion trajectories. 
%In other words, 
As a result, the method provides consistent identity labels in conjunction with accurate segmentations of moving objects.

%
We show that this joint graphical model improves over the individual, task specific models. Our results improve over the state of the art in motion segmentation evaluated on the FBMS59 \cite{Ochs14} motion segmentation benchmark and are competitive on standard multi-target pedestrian tracking sequences \cite{Andriluka:2008:PTD,Zamir:2012:GMC} while additionally providing fine-grained motion segmentations.


==> related.tex <==
\section{Related Work}
Combining high-level cues with low-level cues is an established idea in computer vision
and has been used successfully e.g.\ for image segmentation \cite{DBLP:journals/corr/BertasiusST15}. 
Similarly, motion trajectories have been used for tracking \cite{Fragkiadaki11,FragkiadakiECCV12} 
and object detections for segmenting moving objects \cite{Fragkiadaki_2015_CVPR}. 
However, our proposed method is substantially different in that we provide a unified graph structure whose partitioning both solves the low level problem, here, the motion segmentation task, and the high-level problem, i.e.\ the multi target tracking task, at the  same time. In that spirit, the most related previous work is \cite{FragkiadakiECCV12}, where detectlets, small tracks of detections, are classified in a graphical model that, at the same time, performs trajectory clustering. While we draw from the motivation provided in \cite{FragkiadakiECCV12}, the key difference to our approach is that we cast both, motion segmentation and multi-target tracking, as clustering problems, allowing for the direct optimization of the Minimum Cost Multicuts \cite{chopra-1993,deza-1997}. Thus, we perform bottom-up segmentation and tracking in a single step.

In \cite{milan15}, tracking and video segmentation are also approched as one problem. However, their appoach employs CRFs instead of Minimum Cost Multicuts, is built upon temporal superpixels \cite{tsp} instead of point trajectories and strongly relies on unary terms on these superpixels learned using support vector machines.

In computer vision, Minimum Cost Multicut Formulations have been mainly applied to image segmentation \cite{andres-2011,andres-2012-globally,kappes-2011,keupericcv}. Exceptiontions are \cite{keuper15a} applying this model to motion segmentation and \cite{tang15} applying it to pedestrian tracking. In \cite{tang15}, Minimum Cost Multicuts have shown to provide a suitable alternative to network flow approaches \cite{networkflow1,networkflow2}. The clustering nature of minimum cost multicuts avoids the explicit non-maximum suppression step which is a crucial ingredient in disjoint path formulations such as \cite{networkflow1,networkflow2}.

Different approaches towards solving this combinatorial problem of linking the right detection proposal over time use integer linear programming \cite{Shitrit:2011:TMP,wang-et-al-2014}, MAP estimation \cite{Pirsiavash:2011:GOG}, or continuous optimization \cite{Andriyenko2012CVPR}. In these approaches, the complexity usually needs to be reduced by either applying non-maximum suppression  or pre-grouping detections into tracklets \cite{Huang:2008:ROT,WojekECCV10,AndrilukaCVPR2010,FragkiadakiECCV12,Zamir:2012:GMC,WojekPAMI2013,Henschel:2014:EMP,tang14ijcv}.

%tracking goes there.....
The motion segmentation is, in our framework, cast as a dense point trajectory grouping problem. Related approaches have been suggested in \cite{Bro10c,lezama11,Ochs12,Li2013_12,shiICCV2013,Ochs14,Dragon2014,Ji2014,keuper15a}, most of which employ the spectral clustering paradigm to generate segmentations, while recently \cite{keuper15a} have shown the advantages of casting the motion trajectory segmentation as a minimum cost multicut problem.\\
The approaches of \cite{Cheridata2009,Dragon2012,Bro10c,Ochs14,Li2013_12} base their segmentations on pairwise affinities while \cite{Ochs12,zografos14,Elhamifar2009_6} model higher order motions by different means. In our approach, we do not make use of any higher order motion models. In fact, much of the information these terms carry is already contained in the detections we are using, such that we can leverage this information with pairwise terms. 


